The relativistic velocity addition law optimizes a forecast gambler's profit

We extend the projective covariant bookmaker's bets model to the forecasting gamblers case. The probability of correctness of forecasts shifts probabilities of branching. The formula for the shift of probabilities leads to the velocity addition rule of the special theory of relativity. In the absence of information about bookmaker's wagers the stochastic logarithmic rates completely determines the optimal stakes of forecast gambler.

==> pst-eucl.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% -*- Mode: Latex -*- %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pst-eucl.tex --- Generation of geometric figures in euclidean geometry
%% Copyright 2000-2005 Dominique RODRIGUEZ
%%
%% Author          : Dominique RODRIGUEZ (EN) <dominique.rodriguez@waika9.com>
%% Created the     : Mon Oct 16 21:15:11 CEST 2000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% HISTORY
%%
%% 2000-10-16 : creation of the file from a first LaTeX protype sty file
%%
%% 2001-05-7  : distribution of the first beta version
%%
%% 2002-03-21 : distribution of the second beta version
%%
%% 2002-12-01 : distribution of the pre-release 1.0
%%
%% 2003-03-23 : direct computation of coordinates for the center of gravity and
%%              the center of the circum circle, avoiding creation of intermediates
%%              nodes.
%%
%% 2003-12-16 : Integration of modifications given by Alain DELPLANQUE
%%              automatic computation of PosAngle for several commands,
%%              and ability to give a list of point for pstGeonode, pstOIJGeonode
%%
%% 2004-09-05 : Improvement of the management of the Point name end of the param lists
%%
%% 2004-11-04 : Improvement of the management of the display of the Point name
%%
%% 2004-12-10 : New parameters for coding the circum circle : SegmentSymbolA B & C
%%
%% 2004-12-14 : New parametre RightAngleType for regional difference
%%
%% 2005-01-17 : transition towards pst-xkey (thanks to "Hendri Adriaens" <Hendri@uvt.nl>)
%%
%% 2005-02-21 : correction for spurious blank (thanks to Herbert Voss <Herbert.Voss@alumni.TU-Berlin.DE>)
%%              in pstTriangleABC (search for "-- hv")
%%
%% 2005-03-25 : Modification of the transformations macros: management of a points list
%%              coding for rotation & translation
%%              draw a curve for a points list (geonode & oijgeonode & transform macros)
%%
%% 2005-04-10 : Modification of the transformations macros: management of a points list
%%              management directly within the first point argument
%%              Plotting of a curve linking a list of points
%%
%% 2005-10-09 : problem solved with CodeFigAB
%%
%% 2005-12-31 : use \psscalbox instead of \scalebox (hv)
%%
%% 2006-01-29 : minor changes for file version (hv)
%%
%% 2006-01-30 : correction of pstArcOAB for pscustom (dr)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Require PSTricks and pst-node packages
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\MultidoLoaded\endinput\else\input multido.tex\fi
\def\fileversion{1.3.5}
\def\filedate{2006/01/30}%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
\message{`PST-Euclide v\fileversion, \filedate\space (Dominique RODRIGUEZ)}%
\message{  This version uses the pst-xkey package for managing parameters}%
\message{  Please read the doc, some macros have a new syntax}%
\message{    use option old for upward compatibility}%
\csname PSTEuclideLoaded\endcsname
\let\PSTEuclideLoaded\endinput
%% prologue for postcript
\pstheader{pst-eucl.pro}%
% interface to the `xkeyval' package
\input pst-xkey.tex
\pst@addfams{pst-eucl}
\edef\PstAtCode{\the\catcode`\@}%
\catcode`\@=11\relax
% Definition of the parameters
% ----------------------------
% symbol used for the point
\define@key[psset]{pst-eucl}{PointSymbol}{\edef\psk@PointSymbol{#1}}%
\define@key[psset]{pst-eucl}{PointSymbolA}{\edef\psk@PointSymbolA{#1}}%
\define@key[psset]{pst-eucl}{PointSymbolB}{\edef\psk@PointSymbolB{#1}}%
\define@key[psset]{pst-eucl}{PointSymbolC}{\edef\psk@PointSymbolC{#1}}%
% name used for the point
\define@key[psset]{pst-eucl}{PointName}{\edef\psk@PointName{#1}}%
\define@key[psset]{pst-eucl}{PointNameA}{\edef\psk@PointNameA{#1}}%
\define@key[psset]{pst-eucl}{PointNameB}{\edef\psk@PointNameB{#1}}%
\define@key[psset]{pst-eucl}{PointNameC}{\edef\psk@PointNameC{#1}}%
% use math mode in point name
\newif\ifPst@PtNameMath%
\define@key[psset]{pst-eucl}{PtNameMath}[false]{\@nameuse{Pst@PtNameMath#1}}%
% symbol used for marking equal length segment
\define@key[psset]{pst-eucl}{SegmentSymbol}{\edef\psk@SegmentSymbol{#1}}%
\define@key[psset]{pst-eucl}{SegmentSymbolA}{\edef\psk@SegmentSymbolA{#1}}%
\define@key[psset]{pst-eucl}{SegmentSymbolB}{\edef\psk@SegmentSymbolB{#1}}%
\define@key[psset]{pst-eucl}{SegmentSymbolC}{\edef\psk@SegmentSymbolC{#1}}%
\define@key[psset]{pst-eucl}{Mark}{\edef\psk@Mark{#1}}%
\define@key[psset]{pst-eucl}{MarkAngle}{\edef\psk@MarkAngle{#1}}%
% disance from point to its label
\define@key[psset]{pst-eucl}{PointNameSep}{\edef\psk@PointNameSep{#1}}%
% position angle for positionning a point name
\define@key[psset]{pst-eucl}{PosAngle}{\edef\psk@PosAngle{#1}}%
\define@key[psset]{pst-eucl}{PosAngleA}{\edef\psk@PosAngleA{#1}}%
\define@key[psset]{pst-eucl}{PosAngleB}{\edef\psk@PosAngleB{#1}}%
\define@key[psset]{pst-eucl}{PosAngleC}{\edef\psk@PosAngleC{#1}}%
% dimension of the right angle mark
\define@key[psset]{pst-eucl}{RightAngleSize}{\edef\psk@RightAngleSize{#1}}%
\define@key[psset]{pst-eucl}{RightAngleType}{\edef\psk@RightAngleType{#1}}%
% radius of an angle mark
\define@key[psset]{pst-eucl}{MarkAngleRadius}{\edef\psk@MarkAngleRadius{#1}}%
% angular offset position of the label for marking an angle
\define@key[psset]{pst-eucl}{LabelAngleOffset}{\edef\psk@LabelAngleOffset{#1}}%
% position radius of the label for marking an angle
\define@key[psset]{pst-eucl}{LabelSep}{\edef\psk@LabelSep{#1}}%
% ref point of the label
\define@key[psset]{pst-eucl}{LabelRefPt}{\edef\psk@LabelRefPt{#1}}%
% curve type for point list
\define@key[psset]{pst-eucl}{CurveType}{\edef\psk@CurveType{#1}}%
% coefficient of homothetie
\define@key[psset]{pst-eucl}{HomCoef}{\edef\psk@HomCoef{#1}}%
% angle of rotation
\define@key[psset]{pst-eucl}{RotAngle}{\edef\psk@RotAngle{#1}}%
% label for coding the transfortion
\define@key[psset]{pst-eucl}{TransformLabel}{\edef\psk@TransformLabel{#1}}%
\define@key[psset]{pst-eucl}{CurveType}{\edef\psk@CurveType{#1}}%
% private parameter
\newif\ifPst@CentralSym
\define@key[psset]{pst-eucl}{Central@Sym}[false]{\@nameuse{Pst@CentralSym#1}}%
% for drawing the circum-circle
\newif\ifPst@DrawCirABC
\define@key[psset]{pst-eucl}{DrawCirABC}[true]{\@nameuse{Pst@DrawCirABC#1}}%
% for coding a construction
\newif\ifPst@CodeFig
\define@key[psset]{pst-eucl}{CodeFig}[false]{\@nameuse{Pst@CodeFig#1}}%
\newif\ifPst@CodeFigA
\define@key[psset]{pst-eucl}{CodeFigA}{\edef\psk@CodeFigA{#1}\@nameuse{Pst@CodeFigA#1}}%
\newif\ifPst@CodeFigB
\define@key[psset]{pst-eucl}{CodeFigB}{\edef\psk@CodeFigB{#1}\@nameuse{Pst@CodeFigB#1}}%
\define@key[psset]{pst-eucl}{CodeFigColor}{\edef\psk@CodeFigColor{#1}}%
\define@key[psset]{pst-eucl}{CodeFigStyle}{\edef\psk@CodeFigStyle{#1}}%
\newif\ifPst@CodeFigAarc%
\define@key[psset]{pst-eucl}{CodeFigAarc}[true]{\@nameuse{Pst@CodeFigAarc#1}}
\newif\ifPst@CodeFigBarc%
\define@key[psset]{pst-eucl}{CodeFigBarc}[true]{\@nameuse{Pst@CodeFigBarc#1}}
%% for specifying a distance for the circle
\define@key[psset]{pst-eucl}{Radius}{\edef\psk@Radius{#1}}%
\define@key[psset]{pst-eucl}{RadiusA}{\edef\psk@RadiusA{#1}}%
\define@key[psset]{pst-eucl}{RadiusB}{\edef\psk@RadiusB{#1}}%
\define@key[psset]{pst-eucl}{Diameter}{\edef\psk@Diameter{#1}}%
\define@key[psset]{pst-eucl}{DiameterA}{\edef\psk@DiameterA{#1}}%
\define@key[psset]{pst-eucl}{DiameterB}{\edef\psk@DiameterB{#1}}%
% for specifying a distance for the circle
\define@key[psset]{pst-eucl}{DistCoef}{\edef\psk@DistCoef{#1}}%
\define@key[psset]{pst-eucl}{AngleCoef}{\edef\psk@AngleCoef{#1}}%
% for curvilign abscissa placement
\newif\ifPst@CurvAbsNeg%
\define@key[psset]{pst-eucl}{CurvAbsNeg}[false]{\@nameuse{Pst@CurvAbsNeg#1}}%
% first and last point of a generic curve
\define@key[psset]{pst-eucl}{GenCurvFirst}{\edef\psk@GenCurvFirst{#1}}%
\define@key[psset]{pst-eucl}{GenCurvLast}{\edef\psk@GenCurvLast{#1}}%
% increment of a generic curve
\define@key[psset]{pst-eucl}{GenCurvInc}{\edef\psk@GenCurvInc{#1}}%
%% Default values
% --------------
\psset{%
  PointSymbol=default, PointSymbolA=undef, PointSymbolB=undef, PointSymbolC=undef,
  PointName=default, PointNameA=undef, PointNameB=undef, PointNameC=undef,
  PtNameMath=true, PointNameSep=default, PosAngle=undef, PosAngleA=undef,
  PosAngleB=undef, PosAngleC=undef, Mark=undef, SegmentSymbol=MarkHashh,
  SegmentSymbolA=MarkHashh, SegmentSymbolB=MarkHash, SegmentSymbolC=MarkHashhh,
  RightAngleSize=.4, RightAngleType=default, LabelAngleOffset=0, LabelSep=1,
  LabelRefPt=c, MarkAngle=undef, MarkAngleRadius=.4, HomCoef=.5, RotAngle=60,
  CurveType=none, TransformLabel=none, Central@Sym=false, DrawCirABC=true,
  CodeFig=false, CodeFigColor=cyan, CodeFigStyle=dashed, CodeFigA=undef,
  CodeFigB=undef, CodeFigAarc=true, CodeFigBarc=true, Radius=none, RadiusA=undef,
  RadiusB=undef, Diameter=none, DiameterA=undef, DiameterB=undef, DistCoef=none,
  AngleCoef=none, CurvAbsNeg=false, GenCurvFirst=none, GenCurvLast=none,
  GenCurvInc=1}%}%
\SpecialCoor        %% for using polar coordinates, node position, ...
\psset{dimen=middle}% remark of ML
\def\@undef{undef}%
\def\@default{default}%
\def\@german{german}%
\def\@suisseromand{suisseromand}%
\def\@polygon{polygon}
\def\@polyline{polyline}
\def\@curve{curve}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CORRECTION OF BUG
\def\pst@newnode#1#2#3#4{%
% DG/SR modification begin - Nov.  9, 2000 - Patch 11
  \pst@killglue
% DG/SR modification end
\leavevmode
\pst@getnode{#1}\pst@thenode
\pst@Verb{%
\pst@nodedict
{#3}
\ifx\psk@name\relax false \else \psk@name true \fi
\pst@thenode
#2
{#4}
\tx@NewNode
end}%
\global\let\psk@name\relax
\pstree@nodehook
\global\let\pstree@nodehook\relax}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% list for marking segment
\def\SegSymLst{MarkHash,MarkHashh,MarkHashhh,MarkCros,MarkCross,pstslash,pstslashh,pstslashhh,circ,times,cup,triangle,wedge}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% create a curve after a points list
\def\pst@MngTransformCurve{%DR 25032005
  \ifx\psk@CurveType\@none\else%
  \ifx\psk@CurveType\@polygon\expandafter\pspolygon\@@GenCourbe\else%
  \ifx\psk@CurveType\@polyline\expandafter\psline\@@GenCourbe\else%
  \ifx\psk@CurveType\@curve\expandafter\pscurve\@@GenCourbe%
  \fi\fi\fi\fi}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros for managing a list of parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
       %% begin DR 2005/04/10
\def\@List#1{\xdef\@NewList{none}\@List@i#1,\@nil\ignorespaces}
\def\@List@i#1,{%
\@List@ii#1==\@nil
\@ifnextchar\@nil{\@gobble}{\@List@i}}
\def\@List@ii#1=#2\@nil{%
\ifx\@NewList\@none\xdef\@NewList{#1}\else\xdef\@NewList{\@NewList,#1}\fi}%
       %% end DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@InitListMng{%
  \def\LastValidPN{default}\def\LastValidPNS{default}\def\LastValidPA{undef}\def\LastValidPS{default}}
%%begin modif alaindelplanque 11/2003 (VALID)
%% car(liste) -- param1,param2,... -> param1
\def\PstParamListFirst#1,#2/{#1}
%% cdr(liste) -- param1,param2,... -> param2,...
\def\PstParamListLasts#1,#2/{#2}
\def\Pst@ManageParamList#1{%DR 02092004 #1->point node name
  \edef\OldPointName{\psk@PointName}%
  \edef\psk@PointName{\expandafter\PstParamListFirst\OldPointName,undef/}%
  \ifx\psk@PointName\@undef\edef\psk@PointName{\LastValidPN}\else\edef\LastValidPN{\psk@PointName}\fi
  \edef\OldPointNameSep{\psk@PointNameSep}%
  \edef\psk@PointNameSep{\expandafter\PstParamListFirst\OldPointNameSep,default/}%
  \ifx\psk@PointNameSep\@default\edef\psk@PointNameSep{\LastValidPNS}\else\edef\LastValidPNS{\psk@PointNameSep}\fi
  \edef\OldPosAngle{\psk@PosAngle}%
  \edef\psk@PosAngle{\expandafter\PstParamListFirst\OldPosAngle,undef/}%
  \ifx\psk@PosAngle\@undef\edef\psk@PosAngle{\LastValidPA}\else\edef\LastValidPA{\psk@PosAngle}\fi
  \edef\OldPointSymbol{\psk@PointSymbol}%
  \edef\psk@PointSymbol{\expandafter\PstParamListFirst\OldPointSymbol,undef/}%
  \ifx\psk@PointSymbol\@undef\edef\psk@PointSymbol{\LastValidPS}\else\edef\LastValidPS{\psk@PointSymbol}\fi
  \Pst@geonodelabel{#1}%DR 02092004
  \edef\psk@PointName{\expandafter\PstParamListLasts\OldPointName,undef/}%
  \edef\psk@PointNameSep{\expandafter\PstParamListLasts\OldPointNameSep,default/}%
  \edef\psk@PosAngle{\expandafter\PstParamListLasts\OldPosAngle,undef/}%
  \edef\psk@PointSymbol{\expandafter\PstParamListLasts\OldPointSymbol,undef/}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% create a point with an associated node,
%% #1 -> options
%% #2 -> coordinates
%% #3 -> node name
\def\pstGeonode{\@ifnextchar[\Pst@Geonode{\Pst@Geonode[]}}
\def\Pst@Geonode[#1]{\@ifnextchar({\Pst@Geonode@i[#1]}{\Pst@Geonode@i[#1](0,0)}}
\def\Pst@Geonode@i[#1]{%
  \begingroup%
    \@InitListMng% DR 22032005
    \edef\@@GenCourbe{}%%for accumulating points% DR 22032005
    \psset{#1}\Pst@Geonode@ii}
\def\Pst@Geonode@ii(#1)#2{%
  \pnode(#1){#2}
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points% DR 22032005
  \Pst@ManageParamList{#2}%
  \@ifnextchar(\Pst@Geonode@ii{\pst@MngTransformCurve\endgroup}}% DR 22032005
%%end modif alaindelplanque 11/2003 (VALID)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% create a point with an associated node, in a new
%% landmark
%% #1 -> options
%% #2 -> coordinates
%% #3 -> node name
%% #4 -> O: new center of the landmark
%% #5 -> I: abscissa reference
%% #6 -> J: ordinate reference
\def\pstOIJGeonode{\@ifnextchar[\Pst@OIJGeonode{\Pst@OIJGeonode[]}}%
\def\Pst@OIJGeonode[#1]{%NEW DR 14112001 (for default (0,0) ccordinates)
  \@ifnextchar({\Pst@OIJGeonode@i[#1]}{\Pst@OIJGeonode[#1](0,0)}}%
\def\Pst@OIJGeonode@i[#1]{%
  \begingroup
    \@InitListMng% DR 22032005
    \edef\@@GenCourbe{}%%for accumulating points% DR 22032005
    \psset{#1}\Pst@OIJGeonode@ii}
\def\Pst@OIJGeonode@ii(#1)#2#3#4#5{\Pst@OIJGeonode@iii{#3}{#4}{#5}(#1){#2}}
\def\Pst@OIJGeonode@iii#1#2#3(#4)#5{%
  \rput(#1){%
    \pst@@getcoor{#4}%
    \rput(!\pst@coor\space
      tx@EcldDict begin /N@#2 GetNode /N@#3 GetNode end
      4 index mul 3 -1 roll 5 index mul add
      \pst@number\psyunit dup mul div  exch
      4 -1 roll mul 3 -1 roll 4 -1 roll mul add
      \pst@number\psxunit dup mul div exch){\pnode{#5}}}%
  \xdef\@@GenCourbe{\@@GenCourbe(#5)}%%for accumulating points% DR 22032005
  \Pst@ManageParamList{#5}%
  \@ifnextchar({\Pst@OIJGeonode@iii{#1}{#2}{#3}}{\pst@MngTransformCurve\endgroup}}% DR 22032005
%%end modif DR 11/2003 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% #1 -> point coordinates
\def\Pst@geonodelabel#1{%% {nodename}
  \ifx\psk@PointSymbol\@none\else%
    \ifx\psk@PointSymbol\@default\edef\psk@PointSymbol{*}\fi%
    \psdot[dotstyle=\psk@PointSymbol](#1)%
  \fi%DR 02092004
  \Pst@PutPointLabel{#1}%DR 041104
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Pst@PutPointLabel#1{%DR 041104
  \ifx\psk@PointName\@none\else
    \rput{*0}([nodesep=\ifx\psk@PointNameSep\@default{1em}\else\psk@PointNameSep\fi,
               angle=\ifx\psk@PosAngle\@undef{0}\else\psk@PosAngle\fi]#1)%
      {\ifPst@PtNameMath$\Pst@WhichLabel{#1}$\else\Pst@WhichLabel{#1}\fi}
  \fi}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Pst@WhichLabel#1{\ifx\psk@PointName\@default#1\else\psk@PointName\fi}%DR 0
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% #2 #3 -> nodes defining the segment to mark
\def\pstSegmentMark{\@ifnextchar[\Pst@SegmentMark{\Pst@SegmentMark[]}}%
\def\Pst@SegmentMark[#1]#2#3{%
  \bgroup\psset{#1}%            % Affectation of local parameters
  \ncline[nodesep=0]{#2}{#3}
  \ncput[nrot=:U]{$\csname\psk@SegmentSymbol\endcsname$}%
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% macros for marking
\def\pstslash{/}%
\def\pstslashh{/\!\!/}\let\pstslashslash=\pstslashh%
\def\pstslashhh{/\!\!/\!\!/}\let\pstslashslashslash=\pstslashhh%
%%begin modif alaindelplanque 11/2003
\def\MarkHash{%
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}}
\def\MarkHashh{%
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}(-3\pslinewidth,0)
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}(3\pslinewidth,0)
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}}
\def\MarkHashhh{%
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}(-6\pslinewidth,0)
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}
  \rput{\ifx\psk@MarkAngle\@undef45\else\psk@MarkAngle\fi}(6\pslinewidth,0)
    {\psline(-10\pslinewidth,0)(10\pslinewidth,0)}}
\def\MarkCros{
  \psline(-4\pslinewidth,4\pslinewidth)(4\pslinewidth,-4\pslinewidth)
  \psline(-4\pslinewidth,-4\pslinewidth)(4\pslinewidth,4\pslinewidth)}
\def\MarkCross{
  \psline(-4\pslinewidth,8\pslinewidth)(4\pslinewidth,0)
  \psline(-4\pslinewidth,0)(4\pslinewidth,8\pslinewidth)
  \psline(-4\pslinewidth,-8\pslinewidth)(4\pslinewidth,0)
  \psline(-4\pslinewidth,0)(4\pslinewidth,-8\pslinewidth)}
\def\MarkCirc{\pscircle(0,0){2\pslinewidth}}
%%end modif alaindelplanque 11/2003
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% #2 #3 #4 -> 3 nodes for defining the right angle
\def\pstRightAngle{\@ifnextchar[\Pst@RightAngle{\Pst@RightAngle[]}}%
\def\Pst@RightAngle[#1]#2#3#4{%
  \bgroup\psset{#1}%            % Affectation of local parameters
  %% not good at all, but \rput{0}(#3){\rput{(#2)}{stuff}} doesn't work...
  \rput(#3){%
    \ifx\psk@RightAngleType\@default
    \pspolygon(0,0)%%modif 12/2004
           (!tx@EcldDict begin /N@#4 GetNode exch Atan end \psk@RightAngleSize\space exch PtoC)
           (!tx@EcldDict begin /N@#4 GetNode exch Atan /N@#2 GetNode exch Atan end
              2 copy sub abs 91 gt
                { 2 copy lt { exch 360 add exch } { 360 add } ifelse  } if %%DR 2005/01/14
             %%2 copy lt { exch 360 sub exch } if
              add 2 div 2 sqrt \psk@RightAngleSize\space mul exch PtoC)
           (!tx@EcldDict begin /N@#2 GetNode exch Atan end \psk@RightAngleSize\space
           exch PtoC)
    \else\ifx\psk@RightAngleType\@german
    \pstMarkAngle[MarkAngleRadius=\psk@RightAngleSize,
                  LabelSep=\psk@RightAngleSize\space .5 mul]{#2}{#3}{#4}
       {\psscalebox{\psk@RightAngleSize}{\pscircle*{.08}}}
    \else\ifx\psk@RightAngleType\@suisseromand
    \rput{*0}
      (!tx@EcldDict begin /N@#4 GetNode exch Atan /N@#2 GetNode exch Atan end
        2 copy lt { exch 360 sub exch } if add 2 div .45 \psk@RightAngleSize\space mul exch PtoC)
      {\psscalebox{\psk@RightAngleSize}{\pscircle*{.08}}}
    \pspolygon(0,0)
           (!tx@EcldDict begin /N@#4 GetNode exch Atan end \psk@RightAngleSize\space exch PtoC)
           (!tx@EcldDict begin /N@#2 GetNode exch Atan end \psk@RightAngleSize\space exch PtoC)
    \fi\fi\fi}
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% #2 #3 #4 -> 3 nodes for defining the angle
%% #5 -> label
\def\pstMarkAngle{\@ifnextchar[\Pst@MarkAngle{\Pst@MarkAngle[]}}%
%\def\pstMarkAngle{\@ifnextchar[\Pst@MarkAngle@i{\Pst@MarkAngle@i[]}}%
%\def\Pst@MarkAngle@i[#1]{\@ifnextchar+{\Pst@MarkAngle@ii[#1]}{\Pst@MarkAngle@iii[#1]}}%
%\def\Pst@MarkAngle@ii[#1]+#2#3#4#5{%
%
%%  here we should check the angle size for right angles
%
%}
%\def\Pst@MarkAngle@iii[#1]#2#3#4#5{%
\def\Pst@MarkAngle[#1]#2#3#4#5{%
  \bgroup\psset{#1}%            % Affectation of local parameters
  %\rput(#3){\psarc(0,0){\psk@MarkAngleRadius}{(#2)}{(#4)}}%
  %\rput[\psk@LabelRefPt]%
  %  {*0}([nodesep=\psk@LabelSep, angle= \psk@LabelAngle]#3){#5}%
  \rput(#3){%
    \psarc(0,0){\psk@MarkAngleRadius}{(#2)}{(#4)}%
    \rput[\psk@LabelRefPt]{*0}
      (!tx@EcldDict begin /N@#4 GetNode exch Atan /N@#2 GetNode exch Atan end
        2 copy lt { exch 360 sub exch } if
        add 2 div \psk@LabelAngleOffset\space add \psk@LabelSep\space exch PtoC){#5}
    %%begin modif alaindelplanque 11/2003
    \ifx\psk@MarkAngle\@undef\psset{MarkAngle=90}\fi
    \ifx\psk@Mark\@undef\else
    \rput{!tx@EcldDict begin
            /N@#3 GetNode /N@#4 GetNode ABVect Atan
            /N@#3 GetNode /N@#2 GetNode ABVect Atan
           end 2 copy lt \pslbrace exch 360 sub exch \psrbrace if add 2 div 90 add}
      (0,0){\rput{-90}(\psk@MarkAngleRadius,0){\csname\psk@Mark\endcsname}}
    \fi}
    %%end modif alaindelplanque 11/2003
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% #2 #4 #6 -> coordinates for nodes
%% #3 #5 #7 -> nodes name
\def\pstTriangle{\@ifnextchar[\Pst@Triangle{\Pst@Triangle[]}}%
\def\Pst@Triangle[#1]{%NEW DR 14112001 (for default (0,0) coordinates)
  \def\pst@par{#1}%
  \@ifnextchar(\Pst@Trianglei{\Pst@Trianglei(0,0)}}%
\def\Pst@Trianglei(#1)#2(#3)#4(#5)#6{%
  %\pst@killglue% <------------------------------------------------- hv - DR 050315
  \bgroup\pst@killglue% <------------------------------------------- DR 050315
  %%begin modif alaindelplanque 11/2003
  \pst@@getcoor{#1}\xdef\@@coordi{\pst@coor}%% <-------------------- hv
  \pst@@getcoor{#3}\xdef\@@coordiii{\pst@coor}%% <------------------ hv
  \pst@@getcoor{#5}\xdef\@@coordv{\pst@coor}%% <-------------------- hv
  %%end modif alaindelplanque 11/2003
  %\bgroup\use@par%            % Affectation of local parameters<---- DR 050315
  \use@par%                    % Affectation of local parameters<---- DR 050315
  %%begin modif alaindelplanque 11/2003
  \bgroup\ifx\psk@PosAngleA\@undef
    \psset{PosAngle={!tx@EcldDict begin \@@coordiii\space\@@coordi\space ABVect exch Atan dup
      \@@coordv\space\@@coordi\space ABVect exch Atan exch sub dup abs 180 gt { dup
      dup abs div 360 mul sub } if 2 div add 180 add end}}%% <------ hv
  \else\psset{PosAngle=\psk@PosAngleA}\fi
  %%end modif alaindelplanque 11/2003
  \ifx\psk@PosAngleA\@undef\else\psset{PosAngle=\psk@PosAngleA}\fi
  \ifx\psk@PointSymbolA\@undef\else\psset{PointSymbol=\psk@PointSymbolA}\fi
  \ifx\psk@PointNameA\@undef\else\psset{PointName=\psk@PointNameA}\fi
  \Pst@Geonode@i[](#1){#2}\egroup%%NEW DR 15112001
  %%begin modif alaindelplanque 11/2003
  \bgroup\ifx\psk@PosAngleB\@undef
  \psset{PosAngle={!tx@EcldDict begin \@@coordi\space\@@coordiii\space ABVect exch Atan dup
      \@@coordv\space\@@coordiii\space ABVect exch Atan exch sub dup abs 180 gt { dup
      dup abs div 360 mul sub } if 2 div add 180 add end}}%% <------ hv
  \else\psset{PosAngle=\psk@PosAngleB}\fi
  %%end modif alaindelplanque 11/2003
  \ifx\psk@PosAngleB\@undef\else\psset{PosAngle=\psk@PosAngleB}\fi
  \ifx\psk@PointSymbolB\@undef\else\psset{PointSymbol=\psk@PointSymbolB}\fi
  \ifx\psk@PointNameB\@undef\else\psset{PointName=\psk@PointNameB}\fi
  \Pst@Geonode@i[](#3){#4}\egroup%%NEW DR 15112001
  %%begin modif alaindelplanque 11/2003
  \ifx\psk@PosAngleC\@undef
  \psset{PosAngle={!tx@EcldDict begin \@@coordiii\space\@@coordv\space ABVect exch Atan dup
      \@@coordi\space\@@coordv\space ABVect exch Atan exch sub dup abs 180 gt { dup
      dup abs div 360 mul sub } if 2 div add 180 add end}}%% <------ hv
  \else\psset{PosAngle=\psk@PosAngleC}\fi%% <----------------------- hv
  %%end modif alaindelplanque 11/2003
  \ifx\psk@PosAngleC\@undef\else\psset{PosAngle=\psk@PosAngleC}\fi
  \ifx\psk@PointSymbolC\@undef\else\psset{PointSymbol=\psk@PointSymbolC}\fi
  \ifx\psk@PointNameC\@undef\else\psset{PointName=\psk@PointNameC}\fi
  \Pst@Geonode@i[](#5){#6}%%NEW DR 15112001
  \pst@TraceTriangle{#2}{#4}{#6}%
  \egroup%
}%
\def\pst@TraceTriangle#1#2#3{\pspolygon(#1)(#2)(#3)}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%            Line, circle, Arc
%% #2 #3 -> 2 nodes defining the line
\def\pstLineAB{\ncline}%@ifnextchar[\Pst@LineAB{\Pst@LineAB[]}}%
%\def\Pst@LineAB[#1]#2#3{\ncline[#1]{#2}{#3}}%
%% #2 #3 -> 2 nodes defining the center and a point on the circle
\def\pstCircleOA{\pst@object{pstCircleOA}}%
\def\pstCircleOA@i#1#2{%
  \bgroup\use@par%
  \rput(#1){%
    \begin@ClosedObj
      \def\pst@linetype{4}%
      \addto@pscode{%
        tx@EcldDict begin
          /N@#1 GetNode
          \ifx\psk@Radius\@none
            \ifx\psk@Diameter\@none
              2 copy /N@#2 GetNode ABDist
            \else\psk@Diameter 2 div
            \fi
          \else\psk@Radius\space
          \fi
        end
        \psk@dimen CLW mul sub 0 360 arc closepath}%
      \showpointsfalse
    \end@ClosedObj
  }%
  \egroup%
}%
%% #2 #3 -> 2 nodes defining a diameter of the circle
\def\pstCircleAB{\pst@object{pstCircleAB}}%
\def\pstCircleAB@i#1#2{%
  \bgroup\use@par%
    \Pst@MiddleAB[PointSymbol=none, PointName=none]{#2}{#1}{@MAB}{}
    \rput(#1){%
      \begin@ClosedObj
        \def\pst@linetype{4}%
        \addto@pscode{%
          tx@NodeDict begin
            tx@NodeDict /N@@MAB load GetCenter
          end
          2 copy
          tx@EcldDict begin /N@#2 GetNode ABDist end
          \psk@dimen CLW mul sub 0 360 arc closepath}%
        \showpointsfalse
      \end@ClosedObj
    }%
  \egroup%
}%
%% #2 #3 #4 -> 3 nodes defining the center and two points on the circle
\def\pstArcOAB{\pst@object{pstArcOAB}}%
\def\pstArcnOAB{\pst@object{pstArcnOAB}}%
\def\pstArcnOAB@i{\def\psarc@type{1}\pstArcOAB@i}%
\def\pstArcOAB@i{\pstArcOAB@ii}%\@ifnextchar[\pstArcOAB@ii{\pstArcOAB@ii[]}}%
%OLD%%\def\pstArcOAB@ii#1#2#3{%[#1]#2#3#4{%
%OLD%%  \bgroup\use@par%
%OLD%%  \rput(#1){\pstArcOAB@iii{#2}{#3}}%
%OLD%%  \egroup%
%OLD%%}%
%OLD%%\def\pstArcOAB@iii#1#2%
\def\pstArcOAB@ii#1#2#3{%
  \begin@OpenObj%
    %OLD%%\addto@pscode{\pstArcOAB@iv{#1}{#2} \pstArcOAB@v}%
    \addto@pscode{\pstArcOAB@iv{#1}{#2}{#3} \pstArcOAB@v}%
    \gdef\psarc@type{0}%
    \showpointsfalse
  \end@OpenObj%
}%% end \pstArcOAB@iii
%OLD%%\def\pstArcOAB@iv#1#2%
\def\pstArcOAB@iv#1#2#3{%
  %%\pst@coor /y ED /x ED /r
  %OLD%%0 0 /y ED /x ED /r %%new DR 2005/10/21
  tx@EcldDict begin /N@#1 GetNode end /y ED /x ED /r %%new DR 2005/10/21
  %OLD%%tx@EcldDict begin /N@#1 GetNode end
  tx@EcldDict begin /N@#2 GetNode /N@#1 GetNode ABVect end
  Pyth  def /c 57.2957 r \tx@Div def /angleA
  %OLD%%tx@EcldDict begin /N@#1 GetNode end
  tx@EcldDict begin /N@#2 GetNode /N@#1 GetNode ABVect end
  exch Atan \psk@arcsepA c mul 2 div
  \ifcase \psarc@type add \or sub \fi def
  /angleB
  %OLD%%tx@EcldDict begin /N@#2 GetNode end
  tx@EcldDict begin /N@#3 GetNode /N@#1 GetNode ABVect end
  exch Atan \psk@arcsepB c mul 2 div
  \ifcase \psarc@type sub \or add \fi def
  %ifshowpoints\psarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2 r angleA \tx@PtoC
      y add exch x add exch
      moveto
    \fi
  \fi%
}%% end \pstArcOAB@iv
\def\pstArcOAB@v{%
  x y r angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP } { \ifcase\psarc@type add \or sub \fi }%
    \tx@ArcArrow
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB } { \ifcase\psarc@type sub \or add \fi }%
    \tx@ArcArrow
  \fi
  \ifcase\psarc@type arc \or arcn \fi%
}%% end \pstArcOAB@v
\def\pstArcOAB@showpoints{%
  gsave newpath x y moveto x y r \pst@tempa \pst@tempb
  \ifcase\psarc@type arc \or arcn \fi
  closepath CLW 2 div SLW [ \psk@dash\space ] 0 setdash stroke
  grestore %
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                     HOMOTETHIE
%% #2 -> centre
%% #3 -> antecedent
%% #4 -> node name of the homothetic of #1
\def\pstHomO{\@ifnextchar[\Pst@HomO{\Pst@HomO[]}}%
\expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX %% DR 2005/04/10
\def\Pst@HomO[#1]#2{%
  \bgroup%
  \@InitListMng\def\LastValidSS{default}%%SS means SegmentSymbol
  \psset{#1}\def\@HomCtr{#2}% Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@HomO@i%
}%
\def\Pst@HomO@i#1{%
  \@List{#1}\edef\@antecedentLst{\@NewList}
  \@ifnextchar[\Pst@HomO@ii{\Pst@HomO@ii[default]}%
}%
\def\Pst@HomO@ii[#1]{%
  \@List{#1}\edef\@imageLst{\@NewList}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \Pst@HomO@iii%
}%
\def\Pst@HomO@iii{%
  \ifx\@image\@default\def\@image{\@antecedent '}\fi
  \rput(\@HomCtr){%
    \rput(!
      tx@EcldDict begin /N@\@antecedent\space GetNode end
      \psk@HomCoef\space mul exch \psk@HomCoef\space mul exch
      \pst@number\psyunit div exch \pst@number\psxunit div
      exch){\pnode{\@image}}%
      }%%end rput
  \xdef\@@GenCourbe{\@@GenCourbe(\@image)}%%for accumulating points
  \ifPst@CentralSym\ifPst@CodeFig%
    \edef\psk@OldSegmentSymbol{\psk@SegmentSymbol}%
    \edef\psk@SegmentSymbol{\expandafter\PstParamListFirst\psk@OldSegmentSymbol,undef/}%
    \ifx\psk@SegmentSymbol\@undef\edef\psk@SegmentSymbol{\LastValidSS}\else\edef\LastValidSS{\psk@SegmentSymbol}\fi
    \bgroup%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstSegmentMark{\@image}{\@HomCtr}%
    \pstSegmentMark{\@HomCtr}{\@antecedent}%
    \egroup%
    \edef\psk@SegmentSymbol{\expandafter\PstParamListLasts\psk@OldSegmentSymbol,undef/}%
  \fi\fi%
  \Pst@ManageParamList{\@image}%
  \edef\@antecedentLst{\expandafter\PstParamListLasts\@antecedentLst,undef/}%
  \edef\@imageLst{\expandafter\PstParamListLasts\@imageLst,default/}%
  \edef\@LastValidantecedent{\@antecedent}\def\@LastValidimage{\@image}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}%
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \ifx\@antecedent\@undef\def\@End{\pst@MngTransformCurve\egroup}
  \else\def\@End{\Pst@HomO@iii}\fi%
  \@End%
}%
\else%% OLD SYNTAX
\def\Pst@HomO[#1]#2{%
  \bgroup%
  \@InitListMng\def\LastValidSS{default}%%
  \psset{#1}\def\@HomCtr{#2}% Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@HomO@i-%
}%
\def\Pst@HomO@i-#1#2{%
  \rput(\@HomCtr){%
    \rput(!
      tx@EcldDict begin /N@#1 GetNode end
      \psk@HomCoef\space mul exch \psk@HomCoef\space mul exch
      \pst@number\psyunit div exch \pst@number\psxunit div
      exch){\pnode{#2}}%
      }%%end rput
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points
  \ifPst@CentralSym\ifPst@CodeFig%
    \edef\psk@OldSegmentSymbol{\psk@SegmentSymbol}%
    \edef\psk@SegmentSymbol{\expandafter\PstParamListFirst\psk@OldSegmentSymbol,undef/}%
    \ifx\psk@SegmentSymbol\@undef\edef\psk@SegmentSymbol{\LastValidSS}\else\edef\LastValidSS{\psk@SegmentSymbol}\fi
    \bgroup%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstSegmentMark{#2}{\@HomCtr}%
    \pstSegmentMark{\@HomCtr}{#1}%
    \egroup%
    \edef\psk@SegmentSymbol{\expandafter\PstParamListLasts\psk@OldSegmentSymbol,undef/}%
  \fi\fi%
  \Pst@ManageParamList{#2}%
  \@ifnextchar-{\Pst@HomO@i}{\pst@MngTransformCurve\egroup}%
}%
\fi% END OLD SYNTAX %% DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                   Central Symmetry
%% #2 -> centre
%% #3 -> antecedent
%% #4 -> node name of the symmetrical point of #3
\def\pstSymO{\@ifnextchar[\Pst@SymO{\Pst@SymO[]}}%
\def\Pst@SymO[#1]{\Pst@HomO[SegmentSymbol=\SegSymLst,#1, HomCoef=-1, Central@Sym=true]}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                   Middle of a Segment
%% #2 #3 -> 2 nodes defining the segment
%% #4    -> node name of the middle of [#2 #3]
\def\pstMiddleAB{\@ifnextchar[\Pst@MiddleAB{\Pst@MiddleAB[]}}%
\def\Pst@MiddleAB[#1]#2#3#4{%
  \bgroup\psset{#1, HomCoef=.5}% % Affectation of local parameters
  %%begin modif alaindelplanque 11/2003
  \ifx\psk@PosAngle\@undef% Calcul automatique de PosAngle
    \psset{PosAngle={!tx@EcldDict begin /N@#3 GetNode exch /N@#2 GetNode end
        4 1 roll sub 3 1 roll sub Atan}}
  \fi
  %%end modif alaindelplanque 11/2003
  \expandafter\ifx\csname psteucl@old\endcsname\relax\Pst@HomO[]{#2}{#3}[#4]%
  \else\Pst@HomO[]{#2}{#3}{#4}\fi%%%DR 14042005
  \ifPst@CodeFig%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstSegmentMark{#2}{#4}%
    \pstSegmentMark{#4}{#3}%
  \fi%
  \egroup
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%           Centre of Gravity of a Triangle
%% #2 #3 #4 -> 3 nodes defining the triangle
%% #5       -> node name of the centre of gravity of #2 #3 #4
\def\pstCGravABC{\@ifnextchar[\Pst@CGravABC{\Pst@CGravABC[]}}%
\def\Pst@CGravABC[#1]#2#3#4#5{%
  \bgroup\psset{#1}% % Affectation of local parameters
  \Pst@OIJGeonode@i[](! 1 3 div dup){#5}{#2}{#3}{#4}%DR: 22/03/03
  \egroup
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%           Centre of the circoncrit circle
%% #2 #3 #4 -> 3 nodes defining the triangle
%% #5       -> node name of the centre of the circle
\def\pstCircleABC{\@ifnextchar[\Pst@CircleABC{\Pst@CircleABC[]}}%
\def\Pst@CircleABC[#1]#2#3#4#5{%
  \bgroup\psset{#1}% % Affectation of local parameters
  \rput(#2){%DR: 22/03/03
    \rput(!
      tx@EcldDict begin
        /N@#3 GetNode 2 copy Pyth 3 1 roll exch Atan %Rb Thetab
        dup 3 1 roll %Thetab Rb Thetab
        /N@#4 GetNode 2 copy Pyth 3 1 roll exch Atan %Thetab Rb Thetab Rc Thetac
        3 -1 roll sub dup cos 2 index mul 3 1 roll sin mul %Xb Xc Yc
        dup dup mul 2 index dup mul add 3 -1 roll 3 index mul sub 2 div exch div
        exch 2 div exch 3 -1 roll Rotate
        \pst@number\psyunit div exch \pst@number\psxunit div exch
     end){\Pst@Geonode@i[](0,0){#5}}}%
  %\Pst@InterLL[]{@Middle#2#3}{@Middle#2#3P}{@Middle#2#4}{@Middle#2#4P}{#5}%DR: 22/03/03
  \ifPst@DrawCirABC\pstCircleOA{#5}{#2}\fi
  \ifPst@CodeFig
    \psset{PointSymbol=none, PointName=none, linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle, nodesep=-1}%
    \expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX 14042005
      \Pst@HomO[HomCoef=.5]{#2}{#3}[@Middle#2#3]%
      \Pst@Rotation[RotAngle=90, CodeFig=false]{@Middle#2#3}{#2}[@Middle#2#3P]%
      \Pst@HomO[HomCoef=.5]{#2}{#4}[@Middle#2#4]%
      \Pst@Rotation[RotAngle=90, CodeFig=false]{@Middle#2#4}{#2}[@Middle#2#4P]%
      \Pst@HomO[HomCoef=.5]{#4}{#3}[@Middle#4#3]%
    \else%% OLD SYNTAX
      \Pst@HomO[HomCoef=.5]{#2}{#3}{@Middle#2#3}%
      \Pst@Rotation[RotAngle=90, CodeFig=false]{@Middle#2#3}{#2}{@Middle#2#3P}%
      \Pst@HomO[HomCoef=.5]{#2}{#4}{@Middle#2#4}%
      \Pst@Rotation[RotAngle=90, CodeFig=false]{@Middle#2#4}{#2}{@Middle#2#4P}%
      \Pst@HomO[HomCoef=.5]{#4}{#3}{@Middle#4#3}%
    \fi
    \ncline{#5}{@Middle#4#3}%
    \ncline{#5}{@Middle#2#3}%
    \ncline{#5}{@Middle#2#4}%
    \psset{linestyle=solid}%
    \Pst@RightAngle[]{#5}{@Middle#4#3}{#4}%
    \Pst@RightAngle[]{#5}{@Middle#2#3}{#3}%
    \Pst@RightAngle[]{#5}{@Middle#2#4}{#2}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolA]{#4}{@Middle#4#3}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolA]{@Middle#4#3}{#3}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolB]{#3}{@Middle#2#3}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolB]{@Middle#2#3}{#2}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolC]{#2}{@Middle#2#4}%
    \Pst@SegmentMark[SegmentSymbol=\psk@SegmentSymbolC]{@Middle#2#4}{#4}%
  \fi
  \egroup
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                     TRANSLATION
%% #2 #3 -> 2 nodes defining the translation vector
%% #4 -> antecedent
%% #5 -> node name of the image
\expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX %% DR 2005/04/10
\def\pstTranslation{\@ifnextchar[\Pst@Translation{\Pst@Translation[]}}%
\def\Pst@Translation[#1]#2#3{%
  \bgroup%
  \@InitListMng%
  \psset{#1}\def\@VectorOrigin{#2}\def\@VectorEnd{#3}%
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@Translation@i%
}%
\def\Pst@Translation@i#1{%
  \@List{#1}\edef\@antecedentLst{\@NewList}
  \@ifnextchar[\Pst@Translation@ii{\Pst@Translation@ii[default]}%
}%
\def\Pst@Translation@ii[#1]{%
  \@List{#1}\edef\@imageLst{\@NewList}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \Pst@Translation@iii%
}%
\def\Pst@Translation@iii{%
  \ifx\@image\@default\def\@image{\@antecedent '}\fi
  \rput(\@VectorOrigin){%
    \rput(!
      tx@EcldDict begin /N@\@VectorEnd\space GetNode
      \ifx\psk@DistCoef\@none
      \else\psk@DistCoef\space mul exch \psk@DistCoef\space mul exch\fi
      /N@\@antecedent\space GetNode end
      3 -1 roll add exch 3 -1 roll add exch
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
    {\pnode{\@image}}%
    }%
  \xdef\@@GenCourbe{\@@GenCourbe(\@image)}%%for accumulating points
  \ifPst@CodeFig%
    \bgroup%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \ncline[arrows=->,nodesep=0]{\@antecedent}{\@image}
    \ifx\psk@TransformLabel\@none
    \else
      \ifx\psk@TransformLabel\@default%
        \ncput*{$\ifx\psk@DistCoef\@none\else\psk@DistCoef\fi\overrightarrow{\@VectorOrigin\@VectorEnd}$}
      \else\ncput{\psk@TransformLabel}\fi
    \fi%
    \egroup%
  \fi%
  \Pst@ManageParamList{\@image}%
  \edef\@antecedentLst{\expandafter\PstParamListLasts\@antecedentLst,undef/}%
  \edef\@imageLst{\expandafter\PstParamListLasts\@imageLst,default/}%
  \edef\@LastValidantecedent{\@antecedent}\def\@LastValidimage{\@image}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}%
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \ifx\@antecedent\@undef\def\@End{\pst@MngTransformCurve\egroup}
  \else\def\@End{\Pst@Translation@iii}\fi%
  \@End%
}%
\else%% OLD SYNTAX
\def\pstTranslation{\@ifnextchar[\Pst@Translation{\Pst@Translation[]}}%
\def\Pst@Translation[#1]#2#3{%
  \bgroup
  \@InitListMng%
  \psset{#1}\def\@VectorOrigin{#2}\def\@VectorEnd{#3}%
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@Translation@i-%
}%
\def\Pst@Translation@i-#1#2{%
  \rput(\@VectorOrigin){%
    \rput(!
      tx@EcldDict begin /N@\@VectorEnd\space GetNode
      \ifx\psk@DistCoef\@none
      \else\psk@DistCoef\space mul exch \psk@DistCoef\space mul exch\fi
      /N@#1 GetNode end
      3 -1 roll add exch 3 -1 roll add exch
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
    {\pnode{#2}}%
    }%
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points
  \ifPst@CodeFig%
    \bgroup
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle, nodesep=0}%
    \ncline[arrows=->]{#1}{#2}
    \ifx\psk@TransformLabel\@none
    \else%
      \ifx\psk@TransformLabel\@default%
      \ncput*{\ifx\psk@DistCoef\@none\else\psk@DistCoef\fi$\overrightarrow{\@VectorOrigin\@VectorEnd}$}
      \else\ncput{\psk@TransformLabel}\fi
    \fi%
    \egroup
  \fi
  \Pst@ManageParamList{#2}%
  \@ifnextchar-{\Pst@Translation@i}{\pst@MngTransformCurve\egroup}%
}%
%%%%%%%%%%%%%%%%%%%%%
\fi% END OLD SYNTAX %% DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                     ROTATION
%% #2 -> centre of rotation
%% #3 -> antecedent
%% #4 -> node name of the image
\expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX %% DR 2005/04/10
\def\pstRotation{\@ifnextchar[\Pst@Rotation{\Pst@Rotation[]}}%
\def\Pst@Rotation[#1]#2{%
  \bgroup
  \@InitListMng%
  \psset{#1}\def\@RotCtr{#2}\edef\@@GenCourbe{}%%for accumulating points
  \Pst@Rotation@i%
}%
\def\Pst@Rotation@i#1{%
  \@List{#1}\edef\@antecedentLst{\@NewList}
  \@ifnextchar[\Pst@Rotation@ii{\Pst@Rotation@ii[default]}%
}%
\def\Pst@Rotation@ii[#1]{%
  \@List{#1}\edef\@imageLst{\@NewList}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \Pst@Rotation@iii%
}%
\def\Pst@Rotation@iii{%
  \ifx\@image\@default\def\@image{\@antecedent '}\fi
  \rput(\@RotCtr){%
    \rput(!tx@EcldDict begin /N@\@antecedent\space GetNode \psk@RotAngle\space Rotate end
           \pst@number\psyunit div exch \pst@number\psxunit div exch)%
         {\pnode{\@image}}%
    }%% end \rput
  \xdef\@@GenCourbe{\@@GenCourbe(\@image)}%%for accumulating points
  \ifPst@CodeFig%
    \bgroup
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstArcOAB[arrows=->]{\@RotCtr}{\@antecedent}{\@image}%
    \ncline{\@RotCtr}{\@antecedent}\ncline{\@RotCtr}{\@image}
    \ifx\psk@TransformLabel\@none\else\pstMarkAngle{\@antecedent}{\@RotCtr}{\@image}{$\psk@TransformLabel$}\fi
    \egroup
  \fi%
  \Pst@ManageParamList{\@image}%
  \edef\@antecedentLst{\expandafter\PstParamListLasts\@antecedentLst,undef/}%
  \edef\@imageLst{\expandafter\PstParamListLasts\@imageLst,default/}%
  \edef\@LastValidantecedent{\@antecedent}\def\@LastValidimage{\@image}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}%
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \ifx\@antecedent\@undef\def\@End{\pst@MngTransformCurve\egroup}
  \else\def\@End{\Pst@Rotation@iii}\fi%
  \@End%
}%
%%%%%%%%%%%%%%%%%%%%%
\else%% OLD SYNTAX
\def\pstRotation{\@ifnextchar[\Pst@Rotation{\Pst@Rotation[]}}%
\def\Pst@Rotation[#1]#2{%
  \bgroup
  \@InitListMng%
  \psset{#1}\def\@RotCtr{#2}
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@Rotation@i-%
}%
\def\Pst@Rotation@i-#1#2{%
  \rput(\@RotCtr){%
    \rput(!tx@EcldDict begin /N@#1 GetNode \psk@RotAngle\space Rotate end
           \pst@number\psyunit div exch \pst@number\psxunit div exch)%
         {\pnode{#2}}%
    }%% end \rput
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points
  \ifPst@CodeFig%
    \bgroup
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstArcOAB[arrows=->]{\@RotCtr}{#1}{#2}%
    \ncline{\@RotCtr}{#1}\ncline{\@RotCtr}{#2}
    \ifx\psk@TransformLabel\@none\else\pstMarkAngle{#1}{\@RotCtr}{#2}{$\psk@TransformLabel$}\fi
    \egroup
  \fi%
  \Pst@ManageParamList{#2}%
  \@ifnextchar-{\Pst@Rotation@i}{\pst@MngTransformCurve\egroup}%
}%
\fi% END OLD SYNTAX %% DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%        Intersection between two lines
%% #2 #3 -> nodes defining the first line
%% #4 #5 -> nodes defining the second line
%% #6 -> node name of the image
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstInterLL{\@ifnextchar[\Pst@InterLL{\Pst@InterLL[]}}%
\def\Pst@InterLL[#1]#2#3#4#5#6{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(!
    tx@EcldDict begin
      /N@#2 GetNode /N@#3 GetNode /N@#4 GetNode /N@#5 GetNode InterLines
    end
    \pst@number\psyunit div exch \pst@number\psxunit div exch){\pnode{#6}}%
  \Pst@geonodelabel{#6}%
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Intersection between one line and one circle
%% #2 #3 -> nodes defining the first line
%% #4 #5 -> nodes defining the center and a point onto C
%% #6 -> node name of the first point
%% #7 -> label
%% #8 -> node name of the second point
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstInterLC{\@ifnextchar[\Pst@InterLC{\Pst@InterLC[]}}%
\def\Pst@InterLC[#1]#2#3#4#5#6#7{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(#4){%
    \rput(!
    tx@EcldDict begin
      /N@#2 GetNode /N@#3 GetNode 4 copy EqDr
      \ifx\psk@Radius\@none
        \ifx\psk@Diameter\@none
          /N@#4 GetNode /N@#5 GetNode ABDist
        \else\psk@Diameter 2 div
        \fi
      \else\psk@Radius
      \fi
    InterLineCircle /Glby exch def /Glbx exch def
      \pst@number\psyunit div exch \pst@number\psxunit div exch
    end){\pnode{#6}}%
  \rput(!
    tx@EcldDict begin
      Glbx \pst@number\psxunit div Glby \pst@number\psyunit div
    end){\pnode{#7}}}%
  \bgroup\ifx\psk@PosAngleA\@undef\else\psset{PosAngle=\psk@PosAngleA}\fi%
  \ifx\psk@PointSymbolA\@undef\else\psset{PointSymbol=\psk@PointSymbolA}\fi%
  \ifx\psk@PointNameA\@undef\else\psset{PointName=\psk@PointNameA}\fi%
  \Pst@geonodelabel{#6}\egroup%
  \ifx\psk@PosAngleB\@undef\else\psset{PosAngle=\psk@PosAngleB}\fi%
  \ifx\psk@PointSymbolB\@undef\else\psset{PointSymbol=\psk@PointSymbolB}\fi%
  \ifx\psk@PointNameB\@undef\else\psset{PointName=\psk@PointNameB}\fi%
  \Pst@geonodelabel{#7}%
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Intersection between two circles
%% #2 #3 -> nodes defining the first circle
%% #4 #5 -> nodes defining the second circle
%% #6 -> node name of the first point
%% #7 -> node name of the second point
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstInterCC{\@ifnextchar[\Pst@InterCC{\Pst@InterCC[]}}%
\def\Pst@InterCC[#1]#2#3#4#5#6#7{%
  \bgroup\psset{#1}%        % Affectation of local parameters
  \rput(#2){%
    \rput(!
      tx@EcldDict begin
        \ifx\psk@RadiusA\@undef
          \ifx\psk@DiameterA\@undef
            \ifx\psk@Radius\@none
              \ifx\psk@Diameter\@none
                /N@#3 GetNode Pyth
              \else\psk@Diameter 2 div
              \fi
            \else\psk@Radius\space
            \fi
          \else\psk@DiameterA 2 div
          \fi
        \else\psk@RadiusA\space
        \fi
        \ifx\psk@RadiusB\@undef
          \ifx\psk@DiameterB\@undef
            \ifx\psk@Radius\@none
              \ifx\psk@Diameter\@none
                /N@#4 GetNode /N@#5 GetNode ABDist
              \else\psk@Diameter 2 div
              \fi
            \else\psk@Radius\space
            \fi
          \else\psk@DiameterB 2 div
          \fi
        \else\psk@RadiusB\space
        \fi
        /N@#4 GetNode Pyth InterCircles /N@#4 GetNode
        exch Atan dup /xoC exch def Rotate /Glby exch def /Glbx exch def
        xoC Rotate
      end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)
    {\pnode{#6}}%
    \rput(!
      tx@EcldDict begin
        Glbx \pst@number\psxunit div Glby \pst@number\psyunit div
      end)%
    {\pnode{#7}}%
    }%
  \bgroup\ifx\psk@PosAngleA\@undef\else\psset{PosAngle=\psk@PosAngleA}\fi
  \ifx\psk@PointSymbolA\@undef\else\psset{PointSymbol=\psk@PointSymbolA}\fi
  \ifx\psk@PointNameA\@undef\else\psset{PointName=\psk@PointNameA}\fi
  \Pst@geonodelabel{#6}\egroup%
  \bgroup\ifx\psk@PosAngleB\@undef\else\psset{PosAngle=\psk@PosAngleB}\fi
  \ifx\psk@PointSymbolB\@undef\else\psset{PointSymbol=\psk@PointSymbolB}\fi
  \ifx\psk@PointNameB\@undef\else\psset{PointName=\psk@PointNameB}\fi
  \Pst@geonodelabel{#7}\egroup%
  \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle, arcsep=-1}%
  \ifx\psk@CodeFigA\@undef%
    \ifx\psk@CodeFigB\@undef\ifPst@CodeFig\ifPst@CodeFigAarc\pstArcOAB{#2}{#6}{#7}\else\pstArcnOAB{#2}{#6}{#7}\fi\fi\fi
  \else%
    \ifPst@CodeFigA\ifPst@CodeFigAarc\pstArcOAB{#2}{#6}{#7}\else\pstArcnOAB{#2}{#6}{#7}\fi\fi%
  \fi
  \ifx\psk@CodeFigB\@undef%
    \ifx\psk@CodeFigA\@undef\ifPst@CodeFig\ifPst@CodeFigBarc\pstArcOAB{#4}{#6}{#7}\else\pstArcnOAB{#4}{#6}{#7}\fi\fi\fi
  \else%
    \ifPst@CodeFigB\ifPst@CodeFigBarc\pstArcOAB{#4}{#6}{#7}\else\pstArcnOAB{#4}{#6}{#7}\fi\fi%
  \fi
  \egroup%
}%
%%   Intersection between two functions
%% #2 #3 -> f and g (functions)
%% #4 -> approximation of the root
%% #5 -> node name of the first point
\def\pstInterFF{\@ifnextchar[\Pst@InterFF{\Pst@InterFF[]}}%
\def\Pst@InterFF[#1]#2#3#4#5{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(!
  tx@EcldDict begin
    #4 { #3 } { #2 } NewtonSolving pop
  end){\pnode{#5}}%
  \Pst@geonodelabel{#5}%
  \egroup%
}
%%   Intersection between a function and a line
%% #2 -> f (function)
%% #3 #4 -> points defining the line
%% #5 -> approximation of the root
%% #6 -> node name of the first point
\def\pstInterFL{\@ifnextchar[\Pst@InterFL{\Pst@InterFL[]}}%
\def\Pst@InterFL[#1]#2#3#4#5#6{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(!
  tx@EcldDict begin
    #5 { /N@#3 GetNode /N@#4 GetNode EqDr 1 index div
  \pst@number\psxunit div 3 1 roll div x mul add } { #2 }
  NewtonSolving pop
  end){\pnode{#6}}% 
  \Pst@geonodelabel{#6}%
  \egroup%
}
%%   Intersection between a function and a circle
%% #2 -> f (function)
%% #3 #4 -> points defining the circle (center and point)
%% #5 -> approximation of the root
%% #6 -> node name of the first point
\def\pstInterFC{\@ifnextchar[\Pst@InterFC{\Pst@InterFC[]}}%
\def\Pst@InterFC[#1]#2#3#4#5#6{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(!
  tx@EcldDict begin
    #5 { /N@#3 GetNode 2 copy /N@#4 GetNode ABDist \pst@number\psxunit div
  3 1 roll \pst@number\psyunit div exch \pst@number\psxunit div exch x #2 ABDist sub } { 0 } NewtonSolving pop
  pop dup /x exch def #2
  end){\pnode{#6}}% 
  \Pst@geonodelabel{#6}%
  \egroup%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              ORTHOGONAL PROJECTION
%% #2 #3 -> nodes defining the line where to project
%% #4 -> antecedent
%% #5 -> node name of the image
%% #6 -> label
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX %% DR 2005/04/10
\def\pstProjection{\@ifnextchar[\Pst@Projection{\Pst@Projection[]}}%
\def\Pst@Projection[#1]#2#3{%
  \bgroup%
  \@InitListMng%
  \psset{#1}\def\@FrstPt{#2}\def\@ScdPt{#3}% Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@Projection@i%
}%
\def\Pst@Projection@i#1{%
  \@List{#1}\edef\@antecedentLst{\@NewList}
  \@ifnextchar[\Pst@Projection@ii{\Pst@Projection@ii[default]}%
}%
\def\Pst@Projection@ii[#1]{%
  \@List{#1}\edef\@imageLst{\@NewList}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \Pst@Projection@iii%
}%
\def\Pst@Projection@iii{%
  \Pst@Projection@iv{\@antecedent}{\@image}
  %%begin modif alaindelplanque 11/2003
  %% automatic computation of PosAngle
  \ifx\psk@PosAngle\@undef%
    \psset{PosAngle={!tx@EcldDict begin /N@\@image\space GetNode exch /N@\@antecedent\space GetNode end 4 1 roll
                     sub 3 1 roll sub neg exch atan=20}}
  \fi
  %%end modif alaindelplanque 11/2003
  \xdef\@@GenCourbe{\@@GenCourbe(\@image)}%%for accumulating points
  \Pst@ManageParamList{\@image}%
  \ifPst@CodeFig%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstRightAngle[linestyle=solid]{\@ScdPt}{\@image}{\@antecedent}%
    \ncline{\@antecedent}{\@image}%
  \fi%
  \edef\@antecedentLst{\expandafter\PstParamListLasts\@antecedentLst,undef/}%
  \edef\@imageLst{\expandafter\PstParamListLasts\@imageLst,default/}%
  \edef\@LastValidantecedent{\@antecedent}\def\@LastValidimage{\@image}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}%
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \ifx\@antecedent\@undef\def\@End{\pst@MngTransformCurve\egroup}
  \else\def\@End{\Pst@Projection@iii}\fi%
  \@End%
}%
\def\Pst@Projection@iv#1#2{%
  \ifx\@image\@default\def\@image{\@antecedent '}\fi
  \rput(\@FrstPt){% translation onto #1
    \rput(!tx@EcldDict begin /N@#1 GetNode /N@\@ScdPt\space GetNode Project end
          \pst@number\psyunit div exch \pst@number\psxunit div exch)%
         {\pnode{#2}}%
    }%
}%
%%%%%%%%%%%%%%%%%%%%%
\else%% OLD SYNTAX
\def\pstProjection{\@ifnextchar[\Pst@Projection{\Pst@Projection[]}}%
\def\Pst@Projection[#1]#2#3{%
  \bgroup%
  \@InitListMng%
  \psset{#1}\def\@FrstPt{#2}\def\@ScdPt{#3}% Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@Projection@i-%
}%
\def\Pst@Projection@i-#1#2{%
  \Pst@Projection@ii{#1}{#2}
  %%begin modif alaindelplanque 11/2003
  %% automatic computation of PosAngle
  \ifx\psk@PosAngle\@undef%
    \psset{PosAngle={!tx@EcldDict begin /N@#2 GetNode exch /N@#1 GetNode end 4 1 roll
                     sub 3 1 roll sub neg exch atan=20}}
  \fi
  %%end modif alaindelplanque 11/2003
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points
  \Pst@ManageParamList{#2}%
  \ifPst@CodeFig%
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \pstRightAngle[linestyle=solid]{#1}{#2}{\@ScdPt}%
    \ncline{#1}{#2}%
  \fi%
  \@ifnextchar-{\Pst@Projection@i}{\pst@MngTransformCurve\egroup}%
}%
\def\Pst@Projection@ii#1#2{%
  \rput(\@FrstPt){% translation onto #1
    \rput(!tx@EcldDict begin /N@#1 GetNode /N@\@ScdPt\space GetNode Project end
          \pst@number\psyunit div exch \pst@number\psxunit div exch)%
         {\pnode{#2}}%
    }%
}%
\fi% END OLD SYNTAX %% DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              ORTHOGONAL SYMMETRY
%% #2 #3 -> nodes defining the symmetrical axis
%% #4 -> antecedent node
%% #5 -> node name of the symmetrical point
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\expandafter\ifx\csname psteucl@old\endcsname\relax%% NEW SYNTAX %% DR 2005/04/10
\def\pstOrtSym{\@ifnextchar[\Pst@OrtSym{\Pst@OrtSym[]}}%
\def\Pst@OrtSym[#1]#2#3{%
  \bgroup%
  \@InitListMng%
  \psset{#1}\def\@FrstPt{#2}\def\@ScdPt{#3}%             % Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@OrtSym@i%
}
\def\Pst@OrtSym@i#1{
  \@List{#1}\edef\@antecedentLst{\@NewList}
  \@ifnextchar[\Pst@OrtSym@ii{\Pst@OrtSym@ii[default]}%
}%
\def\Pst@OrtSym@ii[#1]{
  \@List{#1}\edef\@imageLst{\@NewList}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \Pst@OrtSym@iii%
}%
\def\Pst@OrtSym@iii{
  \ifx\@image\@default\def\@image{\@antecedent '}\fi
  \rput(\@FrstPt){% translation onto #1
    \rput(!
      tx@EcldDict begin /N@\@antecedent\space GetNode 2 copy /N@\@ScdPt\space GetNode Project
      /N@\@antecedent\space GetNode ABVect 2 mul 3 -1 roll exch add 3 1 roll 2 mul add exch end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
      {\pnode{\@image}}%
    }%
  \ifPst@CodeFig%
    \bgroup
    \Pst@Projection@iv{\@antecedent}{@ProjOrth\@antecedent on\@FrstPt\@ScdPt}
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \Pst@RightAngle[linestyle=solid]{\@FrstPt}{@ProjOrth\@antecedent on\@FrstPt\@ScdPt}{\@antecedent}%
    \Pst@SegmentMark[]{\@image}{@ProjOrth\@antecedent on\@FrstPt\@ScdPt}%
    \Pst@SegmentMark[]{@ProjOrth\@antecedent on\@FrstPt\@ScdPt}{\@antecedent}%
    \egroup
  \fi%
  \xdef\@@GenCourbe{\@@GenCourbe(\@image)}%%for accumulating points
  \Pst@ManageParamList{\@image}%
  \edef\@antecedentLst{\expandafter\PstParamListLasts\@antecedentLst,undef/}%
  \edef\@imageLst{\expandafter\PstParamListLasts\@imageLst,default/}%
  \edef\@LastValidantecedent{\@antecedent}\def\@LastValidimage{\@image}
  \edef\@antecedent{\expandafter\PstParamListFirst\@antecedentLst,undef/}%
  \edef\@image{\expandafter\PstParamListFirst\@imageLst,default/}
  \ifx\@antecedent\@undef\def\@End{\pst@MngTransformCurve\egroup}
  \else\def\@End{\Pst@OrtSym@iii}\fi%
  \@End%
}%
%%%%%%%%%%%%%%%%%%%%%
\else%% OLD SYNTAX
\def\pstOrtSym{\@ifnextchar[\Pst@OrtSym{\Pst@OrtSym[]}}%
\def\Pst@OrtSym[#1]#2#3{%
  \bgroup%
  \@InitListMng%
  \psset{#1}\def\@FrstPt{#2}\def\@ScdPt{#3}%             % Affectation of local parameters
  \edef\@@GenCourbe{}%%for accumulating points
  \Pst@OrtSym@i-%
}
\def\Pst@OrtSym@i-#1#2{
  \rput(\@FrstPt){% translation onto #1
    \rput(!
      tx@EcldDict begin /N@#1 GetNode 2 copy /N@\@ScdPt\space GetNode Project
      /N@#1 GetNode ABVect 2 mul 3 -1 roll exch add 3 1 roll 2 mul add exch end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
      {\pnode{#2}}%
    }%
  \ifPst@CodeFig%
    \bgroup
    \Pst@Projection@ii{#1}{@ProjOrth#1on\@FrstPt\@ScdPt}
    \psset{linecolor=\psk@CodeFigColor, linestyle=\psk@CodeFigStyle}%
    \Pst@RightAngle[linestyle=solid]{\@FrstPt}{@ProjOrth#1on\@FrstPt\@ScdPt}{#1}%
    \Pst@SegmentMark[]{#2}{@ProjOrth#1on\@FrstPt\@ScdPt}%
    \Pst@SegmentMark[]{@ProjOrth#1on\@FrstPt\@ScdPt}{#1}%
    \egroup
  \fi%
  \xdef\@@GenCourbe{\@@GenCourbe(#2)}%%for accumulating points
  \Pst@ManageParamList{#2}%
  \@ifnextchar-{\Pst@OrtSym@i}{\pst@MngTransformCurve\egroup}%
}%
\fi% END OLD SYNTAX %% DR 2005/04/10
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              mediator line
%% #2 #3 -> nodes defining the segment
%% #4 -> middle of the segment
%% #5 -> node belonging to the mediator line
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstMediatorAB{\@ifnextchar[\Pst@MediatorAB{\Pst@MediatorAB[]}}%
\def\Pst@MediatorAB[#1]#2#3#4#5{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \bgroup
    \ifx\psk@PointSymbolA\@undef\else\psset{PointSymbol=\psk@PointSymbolA}\fi
    \ifx\psk@PointNameA\@undef\else\psset{PointName=\psk@PointNameA}\fi
  %\Pst@HomO[HomCoef=.5]{#2}{#3}{#4}
  \Pst@MiddleAB[]{#2}{#3}{#4}
  \egroup
  \bgroup
    \ifx\psk@PointSymbolB\@undef\else\psset{PointSymbol=\psk@PointSymbolB}\fi
    \ifx\psk@PointNameB\@undef\else\psset{PointName=\psk@PointNameB}\fi
  \expandafter\ifx\csname psteucl@old\endcsname\relax%
    \Pst@Rotation[RotAngle=90, CodeFig=false]{#4}{#3}[#5]%%%DR 26032005
  \else\Pst@Rotation[RotAngle=90, CodeFig=false]{#4}{#3}{#5}\fi%%%DR 14042005
  \egroup
  \ifPst@CodeFig
    \bgroup\psset{linecolor=\psk@CodeFigColor}
    \Pst@RightAngle[]{#3}{#4}{#5}
    \Pst@SegmentMark[]{#2}{#4}\Pst@SegmentMark[]{#4}{#3}%
    \egroup
  \fi
  \ncline{#4}{#5}
  \egroup
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              bissectrice
%% #2 #3 #4 -> nodes defining the angle in #3 anti-clockwise
%% #5 -> node belonging to the bissectrice
%% #6 -> label
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstBissectBAC{\@ifnextchar[\Pst@BissectBAC{\Pst@BissectBAC[]}}%
\def\Pst@BissectBAC[#1]#2#3#4#5{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(#3){%
    \rput(!
      tx@EcldDict begin /N@#4 GetNode exch Atan /N@#2 GetNode end
      2 copy 5 2 roll exch Atan 2 copy lt { exch 360 sub exch } if sub
      2 div tx@EcldDict begin Rotate end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
      {\pnode{#5}}%
    \Pst@geonodelabel{#5}%
    \ncline{#3}{#5}%
    }%% end \rput
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              outside bissectrice
%% #2 #3 #4 -> nodes defining the angle in #3 anti-clockwise
%% #5 -> node belonging to the bissectrice
%% #6 -> label
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pstOutBissectBAC{\@ifnextchar[\Pst@OutBisBAC{\Pst@OutBisBAC[]}}%
\def\Pst@OutBisBAC[#1]#2#3#4#5{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \rput(#3){%
    \rput(!
      tx@EcldDict begin /N@#4 GetNode exch Atan /N@#2 GetNode end
      2 copy 5 2 roll exch Atan 2 copy lt { exch 360 sub exch } if sub
      2 div 90 add tx@EcldDict begin Rotate end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
      {\pnode{#5}}%
    \Pst@geonodelabel{#5}%
    \ncline{#3}{#5}%
    }%% end \rput
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Creation of a point according to a curvilign abscissa
%% #2 -> center of the circle
%% #3 -> point origin of the circle
%% #4 -> point to be placed
\def\pstCurvAbsNode{\@ifnextchar[\Pst@CurvAbsNode{\Pst@CurvAbsNode[]}}%
\def\Pst@CurvAbsNode[#1]#2#3#4#5{%
  \bgroup\psset{#1}%             % Affectation of local parameters
  \Pst@@CurvAbsNode{#2}{#3}{#4}{#5}%
  %%begin modif alaindelplanque 11/2003
  %% \ifx\psk@PointSymbol\@none\else{\Pst@geonodelabel{#4}}\fi%
  \ifx\psk@PointSymbol\@none
  \else
    %% automatic computation of PosAngle
    \ifx\psk@PosAngle\@undef%
      \psset{PosAngle={!tx@EcldDict begin /N@#4 GetNode exch /N@#2 GetNode end 4 1 roll
                        sub 3 1 roll sub neg exch Atan}}
    \fi
    \Pst@geonodelabel{#4}
  \fi%
  %%end modif alaindelplanque 11/2003
  \Pst@geonodelabel{#4}%
  \egroup%
  %% AJOUTER LE MARQUAGE CodeFig
}%
\def\Pst@@CurvAbsNode#1#2#3#4{%
  \rput(#1){%
    \rput(!
      tx@EcldDict begin
        /N@#2 GetNode 2 copy 0 0 ABDist #4 exch div Pi div 180 mul
        \ifPst@CurvAbsNeg neg \fi Rotate
      end
      \pst@number\psyunit div exch \pst@number\psxunit div exch)%
    {\pnode{#3}}%
    }%% end \rput
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%        GENERIC CURVES
%% #2 -> Radical name
%% #3 -> initial counter value
%% #4 -> maximal counter value
\def\pstGenericCurve{\@ifnextchar[\Pst@GenericCurve{\Pst@GenericCurve[]}}%
\def\Pst@GenericCurve[#1]#2#3#4{%
  \bgroup\psset{#1}%       % Affectation of local parameters
    \edef\@@GenCourbe{\ifx\psk@GenCurvFirst\@none\else(\psk@GenCurvFirst)\fi}%
    \pst@cnth=#4
    \advance\pst@cnth by -#3%\@GenCurve% del DR
    \advance\pst@cnth by \psk@GenCurvInc%1 modif DR 020225
    \divide\pst@cnth by \psk@GenCurvInc
    \multido{\i@GenCurve=#3+\psk@GenCurvInc}{\pst@cnth}{%
      \xdef\@@GenCourbe{\@@GenCourbe(#2\i@GenCurve)}}
    \edef\@@GenCourbe{%
      \@@GenCourbe%
      \ifx\psk@GenCurvLast\@none\else(\psk@GenCurvLast)\fi}%
    %\psset{showpoints=true}
    \expandafter\pscurve\@@GenCourbe
  \egroup%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              Parallel line
%% #2 #3 -> nodes defining the line
%% #3 -> antecedent node
%% #4 -> node name of the image
%% #5 -> label
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%              Orthogonal line
%% #2 #3 -> nodes defining the line
%% #3 -> antecedent node
%% #4 -> node name of the image
%% #5 -> label
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Special macros for parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Distance between two points
\def\pstDistAB#1#2{%
  tx@EcldDict begin /N@#1 GetNode /N@#2 GetNode ABDist end
  \ifx\psk@DistCoef\@none\else
    \psk@DistCoef\space mul
  \fi
}
%% Distance specified with a number
\def\pstDistVal#1{
  #1 \pst@number\psxunit mul
  \ifx\psk@DistCoef\@none\else
    \psk@DistCoef\space mul
  \fi
}
%% angle defined by three points
\def\pstAngleAOB#1#2#3{
  tx@EcldDict begin /N@#2 GetNode /N@#3 GetNode ABVect /N@#2 GetNode /N@#1 GetNode ABVect end
  4 copy exch 4 -1 roll mul
  3 -2 roll mul add
  4 -2 roll mul 4 -2 roll mul sub exch Atan
  \ifx\psk@AngleCoef\@none\else
    \psk@AngleCoef\space mul
  \fi
}
%% END: pst-euclide.tex
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

